Sampling Random Spanning Trees Faster than Matrix Multiplication

We present an algorithm that, with high probability, generates a random spanning tree from an edge-weighted undirected graph in $\tilde{O}(n^{4/3}m^{1/2}+n^{2})$ time (The $\tilde{O}(\cdot)$ notation hides $\operatorname{polylog}(n)$ factors). The tree is sampled from a distribution where the probability of each tree is proportional to the product of its edge weights. This improves upon the previous best algorithm due to Colbourn et al. that runs in matrix multiplication time, $O(n^\omega)$. For the special case of unweighted graphs, this improves upon the best previously known running time of $\tilde{O}(\min\{n^{\omega},m\sqrt{n},m^{4/3}\})$ for $m \gg n^{5/3}$ (Colbourn et al. '96, Kelner-Madry '09, Madry et al. '15). The effective resistance metric is essential to our algorithm, as in the work of Madry et al., but we eschew determinant-based and random walk-based techniques used by previous algorithms. Instead, our algorithm is based on Gaussian elimination, and the fact that effective resistance is preserved in the graph resulting from eliminating a subset of vertices (called a Schur complement). As part of our algorithm, we show how to compute $\epsilon$-approximate effective resistances for a set $S$ of vertex pairs via approximate Schur complements in $\tilde{O}(m+(n + |S|)\epsilon^{-2})$ time, without using the Johnson-Lindenstrauss lemma which requires $\tilde{O}( \min\{(m + |S|)\epsilon^{-2}, m+n\epsilon^{-4} +|S|\epsilon^{-2}\})$ time. We combine this approximation procedure with an error correction procedure for handing edges where our estimate isn't sufficiently accurate.

==> arxiv_v2_abstract.tex <==
We present an algorithm that, with high probability, generates a random spanning tree from an edge-weighted undirected graph in $\tilde{O}(n^{4/3}m^{1/2}+n^{2})$ time (The $\tilde{O}(\cdot)$ notation hides $\operatorname{polylog}(n)$ factors). The tree is sampled from a distribution where the probability of each tree is proportional to the product of its edge weights. This improves upon the previous best algorithm due to Colbourn et al. that runs in matrix multiplication time, $O(n^\omega)$. For the special case of unweighted graphs, this improves upon the best previously known running time of $\tilde{O}(\min\{n^{\omega},m\sqrt{n},m^{4/3}\})$ for $m \gg n^{5/3}$ (Colbourn et al. '96, Kelner-Madry '09, Madry et al. '15).

The effective resistance metric is essential to our algorithm, as in the work of Madry et al., but we eschew determinant-based and random walk-based techniques used by previous algorithms. Instead, our algorithm is based on Gaussian elimination, and the fact that effective resistance is preserved in the graph resulting from eliminating a subset of vertices (called a Schur complement). As part of our algorithm, we show how to compute $\epsilon$-approximate effective resistances for a set $S$ of vertex pairs via approximate Schur complements in $\tilde{O}(m+(n + |S|)\epsilon^{-2})$ time, without using the Johnson-Lindenstrauss lemma which requires $\tilde{O}( \min\{(m + |S|)\epsilon^{-2}, m+n\epsilon^{-4} +|S|\epsilon^{-2}\})$ time. We combine this approximation procedure with an error correction procedure for handing edges where our estimate isn't sufficiently accurate.


==> commands.tex <==
% Multiple "thanks" that refer to the same text
% http://tex.stackexchange.com/a/4171
\newcommand*\samethanks[1][\value{footnote}]{\footnotemark[#1]}



% Bold math in bold text
% http://tex.stackexchange.com/a/124311
\makeatletter
\g@addto@macro\bfseries{\boldmath}
\makeatother

% Using the new macro above, we also have to "undo" boldmath for mdseries. Some macros don't use the clean \mdseries to "unbold" text (e.g., amsmath's plain style uses \upshape); thus, it is necessary to modify other macros as well.
\makeatletter
\g@addto@macro\mdseries{\unboldmath}
\g@addto@macro\normalfont{\unboldmath}
\g@addto@macro\rmfamily{\unboldmath}
\g@addto@macro\upshape{\unboldmath}
\makeatother


% A command for "manual" citations which can be useful for providing citations in the abstract of a paper.
% \citem[Text]{key} will insert the citation [Text] and refer to the specified key in the biblography
\DeclareCiteCommand{\citem}
    {}
    {\mkbibbrackets{\bibhyperref{\usebibmacro{postnote}}}}
    {\multicitedelim}
    {}



% Change "plus" symbol for multi-author citations in alphabetic style
% http://tex.stackexchange.com/a/130031
\renewcommand*{\labelalphaothers}{\textsuperscript{+}}



% Change separator for multiple citations to a comma (instead of semicolon)
\renewcommand*{\multicitedelim}{\addcomma\space}



% Remove field "note" from full citations
\AtEveryCitekey{\clearfield{note}}



% Make title in bibliography a clickable link using doi and url information
% https://tex.stackexchange.com/a/146438
%\newcommand{\doiorurl}{%
%  \iffieldundef{doi}
%    {\iffieldundef{url}
%       {}
%       {\strfield{url}}}
%    {http://dx.doi.org/\strfield{doi}}%
%}
%
%\newcommand{\myhref}[1]{%
% \ifboolexpr{%
%   test {\ifhyperref}
%   and
%   not test {\iftoggle{bbx:url}}
%   and
%   not test {\iftoggle{bbx:doi}}
%  }
%  {\href{\doiorurl}{#1}}
%  {#1}%
%}

\newcommand{\myhref}[1]{%
  \iffieldundef{doi}
    {\iffieldundef{url}
       {#1}
       {\href{\strfield{url}}{#1}}}
    {\href{http://dx.doi.org/\strfield{doi}}{#1}}%
}

\DeclareFieldFormat{title}{\myhref{\mkbibemph{#1}}}
\DeclareFieldFormat
  [article,inbook,incollection,inproceedings,patent,thesis,unpublished]
  {title}{\myhref{\mkbibquote{#1\isdot}}}



% Enable line breaks for long links using ocgcolorlinks
% http://tex.stackexchange.com/a/47309
\makeatletter
\AtBeginDocument{%
    \newlength{\temp@x}%
    \newlength{\temp@y}%
    \newlength{\temp@w}%
    \newlength{\temp@h}%
    \def\my@coords#1#2#3#4{%
      \setlength{\temp@x}{#1}%
      \setlength{\temp@y}{#2}%
      \setlength{\temp@w}{#3}%
      \setlength{\temp@h}{#4}%
      \adjustlengths{}%
      \my@pdfliteral{\strip@pt\temp@x\space\strip@pt\temp@y\space\strip@pt\temp@w\space\strip@pt\temp@h\space re}}%
    \ifpdf
      \typeout{In PDF mode}%
      \def\my@pdfliteral#1{\pdfliteral page{#1}}% I don't know why % this command...
      \def\adjustlengths{}%
    \fi
    \ifxetex
      \def\my@pdfliteral #1{\special{pdf: literal direct #1}}% isn't equivalent to this one
      \def\adjustlengths{\setlength{\temp@h}{-\temp@h}\addtolength{\temp@y}{1in}\addtolength{\temp@x}{-1in}}%
    \fi%
    \def\Hy@colorlink#1{%
      \begingroup
        \ifHy@ocgcolorlinks
          \def\Hy@ocgcolor{#1}%
          \my@pdfliteral{q}%
          \my@pdfliteral{7 Tr}% Set text mode to clipping-only
        \else
          \HyColor@UseColor#1%
        \fi
    }%
    \def\Hy@endcolorlink{%
      \ifHy@ocgcolorlinks%
        \my@pdfliteral{/OC/OCPrint BDC}%
        \my@coords{0pt}{0pt}{\pdfpagewidth}{\pdfpageheight}%
        \my@pdfliteral{F}% Fill clipping path (the url's text) with
                           % current color
        %
        \my@pdfliteral{EMC/OC/OCView BDC}%
        \begingroup%
          \expandafter\HyColor@UseColor\Hy@ocgcolor%
          \my@coords{0pt}{0pt}{\pdfpagewidth}{\pdfpageheight}%
          \my@pdfliteral{F}% Fill clipping path (the url's text)
                             % with \Hy@ocgcolor
        \endgroup%
        \my@pdfliteral{EMC}%
        \my@pdfliteral{0 Tr}% Reset text to normal mode
        \my@pdfliteral{Q}%
      \fi
      \endgroup
    }%
}
\makeatother



==> intro.tex <==
	
\section{Abstract}
We present an algorithm for approximately generating random spanning trees on edge-weighted undirected graphs in $\tilde{O}(nm^{2/3}2^{O(\sqrt{\log{n}})})$-time. For unit-weight graphs and $m >> n^{3/2}$, this improves the best previously known running time of $\tilde{O}(\min\{n^{\omega},m\sqrt{n},m^{4/3})$, and reduces the current best running time to $\tilde{O}(\min\{nm^{2/3}2^{O(\sqrt{\log{n}})},m^{4/3})$ [cite]. For general edge-weighted graphs and any edge density, this improves the best previously known running time of $O(n^\omega)$ [cite].


  As in [madry et al], the effective resistance metric will be essential to our algorithm, but we will eschew determinant-based and random walk-based techniques used by previous algorithms. Instead, our algorithm will be Gaussian elimination-based where the Schur complement and it's preservation of effective resistance will play an integral role. Using this fact, we will give a fast algorithm with a combination of recursion, quick approximate computation of Schur complement,  and an error correction procedure. (some of this is copy-pasted from a later section)
	
\section{Introduction}

\todo{sell generating random spanning trees being important}


One of the first major results in the study of spanning trees was Kirchoff's matrix-tree theorem, that showed the total number of spanning trees for general edge weighted graphs was equal to the determinant of the minor of the associated graph Laplacian [cite].

Much of the earlier algorithmic study of random spanning trees heavily utilized these determinant calculations by taking a random integer between 1 and the total trees, then efficiently mapping the integer to a unique tree. This general technique was originally used in by [Guenoche,Kulkarni] to give an $O(mn^3)$-time algorithm, and ultimately was improved to an $O(n^\omega)$-time algorithm by [Colburn et al], where $\omega$ is the exponent associated with the fastest runtime of matrix multiplication. Determinant-based algorithms have the advantage that they can handle edge-weighted graphs, where the weight of a tree is the product of its edge weights. Until our result, $O(n^\omega)$ stood as the fastest algorithm for generating random spanning trees on edge-weighted graphs.

Around the same time as the $O(n^\omega)$-time algorithm was discovered, Broder and Aldous independently showed that spanning trees could be randomly generated with random walks, where each time a new vertex was visited, the edge used to reach that vertex was added to the tree [cite]. Accordingly, this results in an algorithm for generating random spanning trees that runs in the amount of time proportional to the time it takes to cover a graph with a random walk. For general edge-weighted graphs the time to cover a graph can be quite bad, but for unit-weight graphs the cover time tends to be fast, and at worst has an expected running time of $O(nm)$, which improves upon the $O(n^\omega)$-time algorithm for sufficiently sparse graphs.

Kelner and Madry improved upon this result by shortcutting the walk and reducing the expected time to reach all vertices to $\tilde{O}(m\sqrt{n})$. This was the first result to use connections between electrical networks and generating random spanning trees. The algorithm relied on low-diameter graph partitioning, then would contract fully visited low diameter partitions while still preserving the probability of exiting the partition with a certain edge by using fast Laplacian system solvers. 

This was subsequently improved for sufficiently sparse graphs by Madry et al with an algorithm that also uses shortcutting procedures, along with recursive techniques, and has an expected runtime of $\tilde{O}(m^{4/3})$. By introducing a new partitioning technique based upon effective resistance, situations under which low diameter partitions perform poorly are avoided, and combining with the low diameter partition improves the runtime for sufficiently sparse graphs. This algorithm is also the first to introduce recursively finding trees on smaller graphs that correspond to random forests in the original graph, allowing the contraction and deletion of many edges. 

\section{Result}



\todo{should this subsection exist? If so, we probably want to use some of the stuff from the beginning of section 4 (Algorithm). this is just a rough explanation for now}

Our algorithm will use similar recursive techniques to Madry et al, but will have a significantly simpler partitioning process and the smaller graphs will be a result of running approximate Gaussian elimination on all vertices outside of the given partition. More precisely, we will partition the vertices into two sets where each vertex is placed in one of the sets with the same probability $p$, to be specified later.  We will also heavily rely on the effective resistance metric, but it's importance to our algorithm will be the fact that the effective resistance multiplied by the edge weight, which we will call the \textit{leverage score} is exactly the probability that the edge is in a randomly generated spanning tree. At a high level, we can view our algorithm as a sampling process where each edge is randomly placed in the tree based on its current leverage score, and is accordingly contracted or deleted from the graph. Employing the fact that Gaussian elimination preserves effective resistance, we can achieve this sampling process by recursively looking at smaller graphs, where computing the effective resistance of an edge in a small graph is computationally cheap. By running fast, approximate Gaussian elimination, some error will be introduced to the effective resistance, which will be accounted for in an error correction procedure that will occasionally require an expensive computation. 


==> introduction.tex <==

\section{Introduction}

In the past several years, a large body of work has emerged that solves various combinatorial graph problems extremely quickly. These algorithms leverage a number of tools related to solving Laplacian linear systems including fast algorithms for sparsification, effective resistance estimation, and of course, solving the systems themselves \cite{SpielmanTengSolver:journal, KoutisMP10:journal, KoutisMP11, KelnerOSZ13,lee2013efficient, CohenKMPPRX14, KyngLPSS16, KyngS16}. This ``Laplacian Paradigm'' \cite{Teng10} has lead to faster algorithms for max-flow, \todo{etc. add other examples and citations}.

Given the success of these tools, it seems worthwhile to investigate how they may be generalized and improved. Two natural directions for this are
\begin{enumerate}
\item investigating the primitives for Laplacian system solving---do they necessarily have to work the way they do, or are there other ways of providing the same primitives?
\item obtaining faster algorithms for problems related to Laplacian solving that we do not yet have extremely fast algorithms for.
\end{enumerate}

This paper makes progress in both of these directions. Specifically, we
\begin{enumerate}
\item give a fast, novel combinatorial algorithm for estimating all-pairs effective resistances without using the Johnson-Lindenstrauss Lemma \todo{cite}. While there are already fast algorithms for this problem, they all rely on Johnson-Lindenstrauss \todo{verify none of the combinatorial sparsifier papers are able to do this}. %In addition to being interesting in its own right, we hope that By giving a new algorithm that uses different 
\item We give a faster algorithm for the problem of sampling (weighted) spanning trees from (weighted) dense graphs with runtime $\widetilde{O}(n^{5/3} m^{1/3})$. For weighted graphs, this is faster than all prior algorithms for all graph densities. For unweighted graphs, it is faster than all prior algorithms when $m \gtrsim n^{1.75}$. Additionally, it is the first algorithm to beat the current matrix multiplication exponent in dense graphs.
\end{enumerate}

Estimating all-pairs effective resistance is a well-known tool used in certain Laplacian solvers \todo{cite stuff, anything other than Spielman-Teng?} On the other hand, it might not be immediately clear why sampling random spanning trees ought to be viewed as a tool in the same class as Laplacian system solving. There are several ways this view can be justified, but here is one. Every solution to a Laplacian system is a harmonic function with respect to the graph satisfying certain boundary conditions. Harmonic functions on graphs essentially correspond to questions one can ask about random walks. Therefore, it would not be incorrect to say that the information one gains access from solving a Laplacian system is, in a reasonable sense, simply a type of information about random walks on the graph. However, Laplacian systems are not the only questions one can ask about random walks. 
Perhaps the most fundamental algorithmic question concerning random walks is how to efficiently sample one. One interesting question is how to sample a ``loop erased random walk'' between a pair of vertices, which is obtained by doing a random walk from one vertex to the other, then deleting all cycles in chronological order so that the walk becomes a simple path. If one samples this by actually performing a loop erased random walk, this can take a substantial amount of time: in weighted graphs the expected time can be exponential in the description of the problem. As it turns out, however, a loop erased random walk between a pair of vertices can also be sampled by sampling a uniformly random (weighted) spanning tree of the (weighted) graph, then outputting the unique path between the two vertices in the spanning tree.

In short, algorithms for both Laplacian system solving and random spanning tree generation are simply computing different things about random walks in the graph. Therefore, given the great number of applications of Laplacian solvers, there may eventually be a large number of algorithmic applications for generating random spanning trees. While there do not exist many such applications at present---perhaps due in part to the fact that we do not yet have extremely fast algorithms for sampling spanning trees---there are still a handful of applications nonetheless. For example, \todo{cite goyal etal} shows how to use random spanning trees to construct cut sparsifiers, and \todo{cite Madry's atsp paper and Gharan's atsp paper} use the ability to sample weighted spanning trees in order to get an improved approximation algorithm for the asymmetric Traveling Salesman Problem. \todo{apparently the atsp papers require the trees to be weighted, which would be a nice justification for sampling weighted trees, but I've also heard that one might be able to sample from another non-uniform distributition that suffices in nearly linear time. I've emailed Madry asking about this, but I'm not sure I'll get an answer in time for the deadline.}

\subsection{Prior Work}

\todo{add prior work on all-pairs effective resistances, probably cite spielman-teng, also maybe cite combinatorial constructions of spectral sparsifiers and contrast with the fact that they don't get exact ER estimates}

\todo{maybe cite Markov chain algorithms, eg. Jerrum and Son (log sobolev constants for balanced matroids), maybe Feder and Mihael (balanced matroids), maybe broder (same paper that has random walks algorithm also uses it to give polynomial bound of mixing time for markov chain), and maybe some other intermediate papers that made incremental progress between these.}

One of the first major results in the study of spanning trees was Kirchoff's matrix-tree theorem, which states that the total number of spanning trees for general edge weighted graphs is equal to any cofactor of the associated graph Laplacian \cite{Kirchhoff47}.

Much of the earlier algorithmic study of random spanning trees heavily utilized these determinant calculations by taking a random integer between $1$ and the total number of trees, then efficiently mapping the integer to a unique tree. This general technique was originally used in \cite{Guenoche83, Kulkarni90}  to give an $O(mn^3)$-time algorithm, and ultimately was improved to an $O(n^\omega)$-time algorithm by \cite{ColbournMN96}, where $m,n$ are the numbers of edges and vertices in the graph, respectively, and $\omega \approx 2.373$ is the matrix multiplication exponent \cite{Williams12}. These determinant-based algorithms have the advantage that they can handle edge-weighted graphs, where the weight of a tree is defined as the product of its edge weights.\footnote{To see why this definition is natural, note that this corresponds precisely to thinking of an edge with weight $k$ as representing $k$ parallel edges and then associating all spanning trees that differ only in which parallel edges they use.} Despite further improvements for unweighted graphs, no algorithm prior to our work improved upon this $O(n^\omega)$ runtime in the general weighted case in the $25$ years since this work. \todo{If possible, double check with Madry that this statement isn't to strong.} Even for unweighted graphs, nothing faster than $O(n^\omega)$ was known for dense graphs with $m \geq n^{1.78}$.

We now give a brief overview of the improvements for unweighted graphs along with a recent alternative $O(n^\omega)$ algorithm for weighted graphs.

Around the same time as the $O(n^\omega)$-time algorithm was discovered, Broder and Aldous independently showed that spanning trees could be randomly generated with random walks, where each time a new vertex is visited, the edge used to reach that vertex is added to the tree \cite{Broder89, Aldous90}. Accordingly, this results in an algorithm for generating random spanning trees that runs in the amount of time proportional to the time it takes for a random walk to cover the graph. For unweighted this \emph{cover time} is $O(mn)$ in expectation is better than $O(n^\omega)$ in sufficiently sparse graphs and worse in dense ones. However, in the more general case of edge-weighted graphs, the cover time can be exponential in the number of bits used to describe the weights. Thus, this algorithm does not yield any improvement in worst-case runtime for weighted graphs.

Kelner and Madry improved upon this result by showing how to simulate this random walk more efficiently. They observed that one does not need to simulate the portions of the walk that only visit previously visited vertices. Then, they use a low diameter decomposition of the graph to partition the graph into components that are covered quickly by the random walk and do precomputation to avoid explicitly simulating the random walk on each of these components after each is initially covered. This is done by calculating the probability that a random walk entering a component at each particular vertex exits on each particular vertex, which can be determined by solving Laplacian linear systems. This approach yields an expected runtime of $\widetilde{O}(m\sqrt{n})$ for unweighted graphs \cite{KelnerM09}.

This was subsequently improved for sufficiently sparse graphs with an algorithm that also uses shortcutting procedures to obtain an expected runtime of $\widetilde{O}(m^{4/3})$ in unweighted graphs \cite{MadryST15}. Their algorithm uses a new partition scheme based on effective resistance and additional shortcutting done by recursively finding trees on smaller graphs that correspond to random forests in the original graph, allowing the contraction and deletion of many edges. 

Recently, Harvey and Xu~\cite{HarveyX16} gave a simpler deterministic $O(n^\omega)$ time algorithm that uses conditional effective resistances to decide whether each edge is in the tree, contracting the edge in the graph if the edge will be in the tree and deleting the edge from the graph if the edge will not.\footnote{Note that for any edge $e$, there is a bijection between spanning trees of the graph in which $e$ is contracted and spanning trees of the original graph that contain $e$. Similarly, there is a bijection between spanning trees of the graph in which $e$ is deleted and spanning trees of the original graph that do not contain $e$.} Updating the effective resistance of each edge is done quickly by using recursive techniques similar to those in \cite{ColbournDN89} and via an extension of the Sherman-Morrison formula. 



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

